Stateless Reinforcement Learning for Multi-Agent Systems: the Case of Spectrum Allocation in Dynamic Channel Bonding WLANs

Spectrum allocation in the form of primary channel and bandwidth selection is a key factor for dynamic channel bonding (DCB) wireless local area networks (WLANs). To cope with varying environments, where networks change their configurations on their own, the wireless community is looking towards solutions aided by machine learning (ML), and especially reinforcement learning (RL) given its trial-and-error approach. However, strong assumptions are normally made to let complex RL models converge to near-optimal solutions. Our goal with this paper is two-fold: justify in a comprehensible way why RL should be the approach for wireless networks problems like decentralized spectrum allocation, and call into question whether the use of complex RL algorithms helps the quest of rapid learning in realistic scenarios. We derive that stateless RL in the form of lightweight multi-armed-bandits (MABs) is an efficient solution for rapid adaptation avoiding the definition of extensive or meaningless RL states.

==> sections/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{img/authors/sergio_author.png}}]{Sergio Barrachina-Mu\~noz} is a Ph.D. candidate at Universitat Pompeu Fabra (UPF). He received his B.Sc. in Telematics Engineering and M.Sc. in Intelligent Interactive Systems in 2015 and 2016, respectively, both from UPF. He joined the Wireless Networking Research Group in 2015 under the supervision of Dr. Boris Bellalta.  His main research interests are focused on machine learning and data science for next-generation WLANs. 
\end{IEEEbiography}

%\vspace*{-11mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip]{img/authors/alex_author.jpeg}}]{Alessandro Chiumento} is an Assistant Professor in the Pervasive Systems group at the University of Twente, the Netherlands. He received his PhD in Electrical engineering from KU Leuven in 2015. His research interests include reconfigurable networks and cross-layer analysis of wireless systems. He has been working on distributed management solutions for dynamic systems for large and heterogeneous wireless networks. His current interests include softwarised IoT networks, dynamic quality of service, machine learning for wireless and wireless for machine learning.
\end{IEEEbiography}

%\vspace*{-11mm}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.2in,clip,keepaspectratio]{img/authors/boris_author.jpg}}]{Boris Bellalta} is an Associate Professor in the Department of Information and Communication Technologies (DTIC) at Universitat Pompeu Fabra (UPF). He obtained his degree in Telecommunications Engineering from Universitat Polit\`{e}cnica de Catalunya (UPC) in 2002 and the Ph.D. in Information and Communication Technologies from UPF in 2007. His research interests are in the area of wireless networks, with emphasis on the design and performance evaluation of new architectures and protocols. The results from his research have been published in more than 100 international journal and conference papers.\end{IEEEbiography}
	
	\vfill

==> sections/old_sections_14Dec2020/abstract.tex <==
% ----- STUFF FROM THE TARGET JOURNAL ----
%\sergio{Target: Wireless Communications magazine. 4500 words (approx 6 pages double column font 10-pt. Mathematical equations should not be used. In justified cases up to three simple equations may be allowed, provided you have the consent of the Guest Editor. 15 refs}
% Spectrum management is key for WLANs
Spectrum management in the form of primary channel selection and bandwidth allocation is a key factor for the performance of channel bonding wireless local area networks (WLANs).
% CB in standards
%From IEEE 802.11n to more recent standards like 802.11ax and 802.11be, bonding channels together is permitted to increase transmissions’ bandwidth. While such an increase favors the potential network capacity, it comes at the price of reduced power per Hertz and accentuated issues on contention and interference with neighboring nodes.
% Heuristics as a possible solution
Traditional spectrum management solutions relying on pre-fixed rules or heuristics are deeply tied to the meaningfulness of the gathered observations (e.g., mean channel occupancy in a certain time window), and are normally appropriate for steady deployments since observations rapidly become outdated in dynamic scenarios.
% ML is needed
To cope with the varying environments imposed by multi-agent systems, where networks change their configurations at their own, the wireless community is experiencing a change of paradigm towards solutions aided with machine learning (ML), and especially reinforcement learning (RL) given its ability to adapt to the system trough a trial-and-error approach.  %\bcom{Why? Is ML giving hopes to deal with this multi-agent scenario?} \sergio{Yes, ML is supposed to tackle complex systems, including multi-agent setups. Should we explicit that with another sentence?} \bcom{If it's possible to say 'how' in a sentence, I would like to find it as a reader.} \sergio{I don't think we can state how in a single sentence since the "how" depends on the problem (architecture, communication, goal...). That is, there are different ML approaches to solve different problems. We may rely on a simple sentence like "due to its ability to adapt to complex systems" or something like this.}
However, strong assumptions are normally made in the context of spectrum management in order to let complex RL models converge to near-optimal solutions.
% Other solutions use DRL
Our goal with this paper is two-fold: justify in a comprehendible way why RL should be the approach for wireless networks problems like spectrum management, and call into question whether the use of complex RL algorithms really helps the quest of rapid learning in realistic scenarios. As for the latter, we derive that stateless RL, especially in the form of lightweight multi-armed-bandits (MABs), is an efficient solution for rapid adaptation avoiding the definition of extensive or meaningless states.

==> sections/old_sections_14Dec2020/future.tex <==
%\section{Challenges and future directions}
\section{Concluding remarks}

% Summary of this paper
In this paper we postulate MABs as an efficient ready-to-use formulation for spectrum management in multi-agent channel bonding WLANs. Apart from highlighting their higher performance with respect to heuristic approaches as for learning better configurations, we delve deep on why more complex RL approaches relying on states do not suit the problem in terms of fast adaptability.

% Other pending tasks
% Some conclusion
In this regard, we envision the use of states for larger time horizons when the focus is not put on rapid-adaptation but on reaching higher potential performance in the long-run. Hereof, we believe that using MABs for generating training datasets to be later fit in more complex ML models is an interesting venue for research. Finally, we leave the design of advanced channel allocation mechanisms that consider the use of domain knowledge-empowered MABs for future work.

% In this regard, we envision the use of states for larger time horizons when the focus is not put on rapid-adaptation but on reaching higher potential performance in the long-run. Hereof, we believe that using MABs for generating training datasets to be later fit in more complex ML models is an interesting venue for research\bb{, since there is the tradeoff between exploiting good actions and exploring random configurations to enhance the dataset.} Finally, we leave the design on customized MABs based on the spectrum management's domain knowledge as future work. \bcom{I posar això: Finally, we leave the design of advanced channel allocation mechanisms that consider the use of MABs for future work.}

% Key concepts for future work
% 1 - states for long-term RL in the background. E.g., a DQN that trains for several days/weeks
% 2 - MABs could be also thought for generating the dataset to be fit Deep RL but also to other categories like SL or UL
% 3 - Customized MABs through the use of the domain knowledge of WiFi. 

==> sections/old_sections_14Dec2020/introduction.tex <==
\section{Introduction} \label{section:introduction}

% Motivation: WLANs and its ever-increasing performance needs
State-of-the-art wireless applications like augmented reality, virtual reality, or 8K video streaming are urging next-generation wireless local area networks (WLANs) to support ever-increasing demands on performance. Among the different approaches to enhance spectrum management in WLANs, channel bonding at the 5 GHz band was introduced in 802.11n-2009 for bonding up to 40 MHz, and further extended in 802.11ac/ax and in 802.11be to bond up to 160 and 320 MHz, respectively. 

% Scarcity of spectrum is the main problem
However, spectrum efficiency has been an increasing issue since the conception of Wi-Fi. 
% Scenarios
In particular, in uncoordinated WLAN scenarios like domestic networks in dense urban areas, dynamics are normally complex and difficult to prevent beforehand due to their rivalry and sometimes chaotic nature.
% Complexity
Essentially, \mbox{Wi-Fi} operates at the industrial, scientific and medical (ISM) band, so anybody can create a new basic service set (BSS) at convenience by occupying one (or multiple) channels inside the \mbox{Wi-Fi} channelization. Further, the channel accesses are attempted at random as mandated by the backoff procedure of the distributed coordination function. These factors generate uncertain contention and interference that is further exacerbated when implementing channel bonding schemes~\cite{deek2013intelligent}. So, even though a recent study shows that the 5 GHz Wi-Fi band remains under-utilized \cite{barrachina2020wifi}, there are peaks in the day where chunks of the spectrum are already getting crowded. This fact, especially in the high-density deployments to come in the next years, leads to different well-known problems like hidden and exposed nodes, ultimately hindering Wi-Fi's performance.

% Fast adaptation
To provide the users with good quality of service in such complex scenarios, fast adaptation is a must for supporting highly demanding applications. To that aim, BSS's must find satisfactory configurations \textit{as soon as possible}. % Heuristics are limited
In this regard, there are many valuable works in the literature about spectrum management proposing custom channel allocation and channel bonding solutions in wireless networks relying on heuristics (e.g., \cite{zheng2014stochastic}). Heuristics are low-complex problem-solving methods that work well in steady scenarios. However, in dense and dynamic scenarios, its performance is severely undermined since they rely on statistics only from recent observations that tend to be outdated when applied. So, heuristics are limited to the meaningfulness of the gathered observations because the same observation-action pairs are always applied, no matter its past performance, thus overlooking potentially better actions selection.

%\bcom{Is this not applying also to RL methods?} \sergio{Yes, it is. That's why I say "only", to emphasize the fact that heuristics normally depend on what happens "now". Instead, RL is able to get a broader picture. I propose putting a clarification in Sec II-B and briefly compare heuristics vs RL.} \bcom{Following Alex's comment, why not providing a definition of heuristics that suits better our interests: i.e., a sequence of pre-defined actions? I agree we should enforce the idea of 'pre-defined' set of actions for any situation vs 'learning the best actions' so we can adapt to any case. Talking about 'observations' makes me (and likely the readers too) think to much on the ability of learning also for heuristics.} \sergio{well, I don't think they are predefined. They are based on what they see. E.g., to go from A to B, hop to the closest neighbor.}

% RL to the rescue. MABs the best
To overcome heuristics' limitations, we first motivate the need of machine learning (ML) to tackle the joint problem of primary and secondary channels allocation in dynamic channel bonding WLANs. Then, we address why supervised and unsupervised learning are not suitable for the problem given the need for fast adaptation in uncertain environments where it is not feasible to train enough to generalize. In this regard, we envision reinforcement learning (RL) as the only ML candidate to achieve the intended purpose
%\bcom{Not sure if the purpose is clear enough. Since relevant, I would state it explicitly, as different readers may understand different things} \sergio{We want to quickly adapt to the environment no matter the model behind, i.e., we don't care about generalizing to unknown systems, right? What would be the purpose?} \bcom{Clear!}
, which is not aimed to generalize to unknown deployments but to quickly adapt to particular (most of the times unique) scenarios. 
% What is RL and the framework we propose
We then justify why stateless RL formulations and, in particular, multi-armed bandits (MABs) suit better to the problem in front of temporal difference variations like Q-learning. As well, we call into question the usefulness of deep reinforcement learning (DRL) due to the unfeasible amount of data it needs to learn. Notice that the reasoning presented in this paper is valid for other problems beyond spectrum management, such as spatial reuse or scheduling.

% What is different in this paper?
%Other papers in the literature leverage RL techniques for spectrum management in wireless networks. However, such works rely on different strong assumptions that can result in inaccurate or even missleading conclusions. In contrast, we explore the performance of RL in much more challenging and realistic scenarios by capturing both physical and medium access control (MAC) dynamics, and stochastic buffering. By means of simulations through the Komondor wireless network simulator~\cite{barrachina2019komondor}, this work is the first one in assessing the performance of RL algorithms in potentially overlapping WLANs with actual IEEE 802.11ac/ax channel bonding capabilities. 

% Holistic scenario
Finally, we present a self-contained toy use-case to compare the performance of a simple stateless MAB formulation based on $\epsilon$-greedy against the well-known Q-learning relying on states, and a contextual variation of $\epsilon$-greedy. Extensive simulation results show that the MAB outperforms the rest both in terms of learning speed and mid/long-term performance. These results suggest that deploying lightweight MAB algorithms in uncoordinated deployments like domestic access points (APs) would boost the network performance through fast adaptation to the environment.


==> sections/old_sections_14Dec2020/mapping_rl.tex <==
\section{Mapping the problem to RL}

% OLD 

% Intro to the section
This section depicts the modifiable attributes, actions, and system statuses composing the learning framework for the primary channel and maximum bandwidth allocation in dynamic channel bonding WLANs. Notice that by defining the primary channel and maximum bandwidth, we actually determine the secondary channels since we follow the IEEE 802.11ac/ax channelization. We then formally formulate the problem to solve.


% --------
% Actions
% --------
\subsection{Attributes and actions}    \label{sec:actions}

% Primary channel and max bw are important
While it is clear that the primary channel is critical to the BSS performance since it is where the backoff procedure runs, the maximum bandwidth is of significant relevance as well. Indeed, once the backoff expires, the channel bonding policy and maximum allowed bandwidth will determine the basic channels to transmit in. Notice that limiting the bandwidth, or being conservative in general, may be much appropriate to BSS's in order to reduce adverse effects like unfavorable contention or hidden nodes.
%
Hence, given the relevance of the primary channel and the maximum bandwidth, we consider two configurable attributes each agent-empowered AP can modify during the learning process:
\begin{itemize}
    %
    \item \textbf{Primary channel} $\boldsymbol{p}$: primary channel where the backoff procedure is executed, $p \in \{1,2,3,4\}$.
    %
    \item \textbf{Maximum bandwidth} $\boldsymbol{b}$: maximum bandwidth (in number of basic channels), $b \in \{1, 2, 4\}$. Recall that, with dynamic channel bonding, the transmitter can adapt to the sensed spectrum on a per-frame basis. So, the bandwidth limitation just sets an upper bound on the number of basic channels to bond.
    %
\end{itemize}
%

Therefore, each BSS encounters an action space $\mathcal{A}$ of size $4 \times 3 = 12$, where actions (or spectrum configurations) have the form $a = (p,b) \in \mathcal{A}$. Should we consider a central single agent managing multiple BSS's, the central action space would increase exponentially with the number of controlled BSS's.



% --------
% Status and states
% --------
\subsection{About statuses, observations and states}

Before introducing what is an \textit{state}%\bcom{I would not use discussing here. Introducing sounds better for me. However, since at the end, we say it depends on the RL algorithm... I would maybe just talk about statuses in this subsection} \sergio{I would keep statuses and states altogether to clearly differentiate them}
, which its definition highly depends on the design of the RL framework, let us coin a new concept called system \textit{status} to depict how the whole WLAN \textit{looks like} at time $t$. the system status $\mathcal{H}_t$ is the minimum \textit{information} we need to describe the entire WLAN in a given time instant $t$. 
%
The system status $\mathcal{H}_t$ of a WLAN deployment with $W$ agent-empowered BSS's at time $t$ is given by three key parameters of each BSS $w$ in the WLAN, like if we were taking a screenshot of the system: the primary channel $p_{w,t}$, the maximum bandwidth $b_{w,t}$, and the quantized mean load $\ell_{w,t}$. Formally, a status is defined by the $\mathcal{H}_t = \{(p_{1,t},b_{1,t},\ell_{1,t}), (p_{2,t},b_{2,t},\ell_{2,t}), ...,(p_{W,t},b_{W,t},\ell_{W,t})\}$.

% Rely on quantization of load
Notice that we could rely on a quantization of the mean traffic load $\ell$ to discretize its continuous domain. Further, notice that the agent cannot modify the load $\ell$ by any means since it is application-dependent. Naturally, the throughput performance depends on the traffic load, the AP configuration, and the rest of BSS's configurations and loads. 
% Size of status
Finally, the amount of possible statuses a certain deployment may have is given by the possible values each of the status parameters can take, which raises again exponentially with the number of agents and size of the attributes' spaces.

Naturally, most of the time, the agents cannot know the system's status in a real-time fashion. However, they could rely on partial and delayed observations to then infer the most accurate state through some discretization function. Besides, since observations are architecture-dependent -- given they may be limited to local sensing capabilities or, on the contrary, be shared via a central controller -- the states' definition is also strictly dependent on the RL framework under consideration.% As later exposed in Section \S\ref{sec:rl_approaches}, we will rely on MABs, where no states are required, and just pairs action-reward are used.

% --------
% Problem definition
% --------
\subsection{Problem definition}

% Intro
In general terms, our goal %for this use-case
is to improve the BSS's performance by maximizing their throughput. %\bcom{The use-case has not been introduced yet}
The key then is to let the BSS's find (learn) the best actions $(p,b)$, where \textit{best} depends on the problem formulation itself.
% Goal of this work is general
We define the throughput satisfaction $s$ of a BSS at iteration $t$ simply as the ratio of throughput to generated traffic load in that iteration. The throughput satisfaction is a commonly used parameter to indicate the ratio of packets acknowledged to the number of packets generated by a BSS in a given time window. Thus, a satisfaction value $s=1$ indicates that all the traffic has been successfully received at the destination.

% Reward
Once the main performance metric has been defined, we may formulate the reward function $R$, the philosopher stone of any RL algorithm. For simplicity, we define $R\equiv s$ given that the throughput is bounded per definition from 0 to 1, which is convenient for guaranteeing convergence in most RL algorithms.
% Problem definition
Regardless of the reward function $R$, we aim at maximizing the cumulative reward \textit{as soon as possible}, $G = \sum_{t=1}^{T}r_t$, where $T$ is the number of iterations we have to execute the learning, and $r_{t}$ is the reward at iteration $t$. Let us emphasize the complexity of the problem by noting that $r_{t}$ depends on the reward definition $R$, on the action $a_t$ selected at $t$, and also on the system status $\mathcal{H}_{t}$.

%\bcom{I would made emphasis in the introduction on the need to find a solution as soon as possible. Not sure it is clearly stated there.} \sergio{Ok. Proposal made in Intro.}

==> sections/old_sections_14Dec2020/ml.tex <==
\section{A change of paradigm towards reinforcement learning}

%% OLD 

% Why heuristics may be not enough
Heuristics are deeply tied to the meaningfulness of recent observations, and such meaningfulness is hard to maintain when the environment changes. Then, in uncoordinated, high-density deployments, where multiple BSS's adapt their spectrum configurations at their own, designing accurate hand-crafted spectrum management techniques is unfeasible.

%\bcom{Is this a good example of heuristics? When this heuristic is executed? Continuously? Every X minutes? If its continuously, why it is not able to adapt? I would present the problem of heuristics as the fact they are not able to find an (implicit) agreement between agents. If space, I would add an example of why an heuristic is not working, it will help a lot readers to understand the problem.} \sergio{\textbf{Propsal made below}}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{img/example_heuristic.pdf}
    \caption{A toy example where throughput maximizing heuristics fall into detrimental loops. The primary channel in each iteration is highlighted with bold text for both BSS's.}
    \label{fig:example_heuristic}
\end{figure}

To illustrate the pitfalls of heuristic approaches, let us depict a toy scenario with two potentially overlapping BSS's with dynamic channel bonding capabilities, A and B, in a system of 4 channels following the IEEE 802.11ac/ax channelization. Assume also that both BSS's continuously require at least 40~MHz of free spectrum to be satisfied. Therefore, by allocating channels 1 and 2 to one BSS and channels 3 and 4 to the other, the problem would be solved. However, in decentralized multi-agent settings, it is up to the BSS's to find satisfactory configurations. A possible heuristic in this case could be relying on the primary channel selection that is expected to provide higher throughput given the occupancy of both the target primary and the neighboring secondary channels~\cite{barrachina2019online}. In this case, a BSS would periodically measure the spectrum occupancy at all the channels. After each monitoring period, the BSS would switch to another primary if not satisfied with current performance. For instance, BSS A, starting with primary channel 2 would switch to channel 3 or 4 with same probability given that both were free during period 1, so they are likely to be good candidates to increase the throughput by bonding them. However, since BSS B also determines that switching from primary channel 1 to 3 would be beneficial as well, a loop is started where heuristics do not work.\footnote{Note that it is not necessary to have synchronous BSS's to fall into the loop given both use the same observation time per iteration.} This occurs because observations are outdated from one period to the other and action selection is never based on past performance, thus disregarding any learning.

% Are there alternatives? Yes, ML. Trend to ML in the community
With this simple example, we have seen that heuristics, even for petite deployments, may be detrimental to performance. So, are there alternatives to pre-fixed rules algorithms and heuristics? Indeed, ML solutions have been widely studied in wireless networks for a plethora of problems. The capability of ML for going beyond rule of thumb strategies by automatically learning (and adapting) to (un)seen situations can cope with heterogeneous scenarios, including  different mobility, connectivity, and performance requirements. That is, a change of paradigm towards solutions aided with ML is getting increasingly common in the context of present and future wireless networks~\cite{luong2019applications,zappone2019wireless}.

% Why previous SoA on our problem is limited in the sense of not using ML
%As for the joint problem of channel allocation and channel bonding, multi-channel next-generation WLANs' complex dynamics will make it necessary to rely on some sort of learning to overcome hand-crafted alternatives. That is, relying on prior hard-coded rules and protocols seems not an option in the quest to support the ever-increasing demands of next-generation services and applications in terms of very high throughputs and very low delays. Further, undertaking new protocol designs that could consider all the dynamism and generalize to a complete set of scenarios is merely hopeless.

% - What is reinforcement learning
\subsection{What is reinforcement learning?}

% What is RL in plain words
% from https://deepsense.ai/what-is-reinforcement-learning-the-complete-guide/
RL refers to sequentially training ML models based on decisions taken towards maximizing a cumulative reward. RL relies on agents that ought to learn how to achieve a goal in an uncertain, potentially complex environment. The agent employs trial and error to come up with a solution to the problem. To get the agent to do what the programmer (or administrator) wants, the agent gets either rewards (e.g., throughput) or penalties (e.g., delay) for the actions it performs (e.g., switch to another primary channel). Its goal is to maximize the total reward (e.g., mean throughput during an observation time). Although the designer sets the reward function and policy, i.e., the rules of the game (e.g., the higher throughput, the better), he/she gives the model no hints or suggestions for how to approach the game. %\bcom{Solving the game is what is said in the next sentence?} \sergio{Well, it depends on the definition of solving. RL just proposes a approach to try to get the most reward, while it may not be optimal.}. \bcom{I agree. Indeed, the comment was related to if it was necessary to link better the two sentences}
It is up to the RL algorithm to figure out how to perform the task to maximize the reward, normally starting from random trials and finishing with sophisticated tactics.

% RL and WLANs
More formally, RL models an agent that tries to learn how to behave in an environment by performing actions and observing the collected rewards. At a given iteration $t$, action $a$ results in a reward observation drawn from a reward distribution $r_t(a) \sim \theta_a$. In the context of WLANs, an agent could be installed into an AP that tries to maximize a certain BSS performance metric by testing different configuration settings and adapting to the collected reward observations through trial-and-error.

% - Why RL and not other ML frameworks?
\subsubsection{Model-based vs. model-free}
% Model-based vs. model-free
There are two main RL approaches: \textit{i}) \textbf{model-based approach} to first estimate the system model from observations and then apply dynamic programming or a computationally efficient heuristic policy such as myopic or Whittle index policies, and \textit{ii}) \textbf{model-free approach} to learn the policy directly through interactions with the system without estimating the system model. The model-based approach is less favored for our problem since the agent’s limited observation capability may result in a bad (and most times outdated) system model estimation. %bcom{is not the same problem with heuristics?} \sergio{Well, it is in the sense that misleading observations are detrimental. However, the model-based RL approach tries to learn the model to later define the best strategy. Heuristics are already strategies from its conception.}

% We must rely on model-free
In particular, since system interactions in problems like spectrum management are critically complex and generated by multiple actors (i.e., wireless devices), it is often preferable to rely on model-free approaches. That is, when getting rid of strong assumptions like Markovian channels% (e.g., \cite{dai2014online}) \bcom{is it worth to waste a reference for this?}
, it would not make sense to have an agent trying to infer what is the model behind the interactions perceived at the varying power levels detected at each of the channels. Moreover, even in the case where such interference model was stationary (and let us also assume simple enough to be accurately captured through a model), in the very moment that the agent-empowered AP initiated a transmission, the contention and interference generated to surrounding nodes may completely change the learned model consequently. Thus, one can easily derive that having a giant model considering all the possibilities, or a specific model per each configuration, is merely unpractical.%\bcom{sounds dramatic... maybe too much for a technical paper.} \sergio{unpractical/unfeasible rather than hopeless?}. \bcom{unpractical sounds better, I guess}

% - Why RL and not other ML frameworks?
\subsection{Why RL and not other ML categories?}

%In plain words, RL seems to fit more naturally to the spectrum management problem than the other two principal ML alternatives: supervised learning (SL) and unsupervised learning (UL). We reason why below. \bcom{I feel this paragraph does not gives much information. Do we need a paragraph introducing this subsection?}
Heuristics fall in multi-agent settings since they rely on current observations, which are normally misleading when the environment changes frequently. RL tries to tackle that but looking at the big picture. So, even though observations can be misleading as well, RL relies on the learning performed through historical pairs state/action-reward, generating action selections beyond current observations.
%
However, why should RL be the ML category of choice? We next justify what the other to big ML categories are unpractical for this type of problems.

%\subsubsection{Supervised Learning}

% What is SL
\textbf{Supervised learning (SL)} is the ML task of learning a function that maps an input $x$ to an output $y$ based on example input-output pairs $(x_i, y_i)$. It estimates a function from labeled training data consisting of a set of training examples. An SL algorithm then analyzes the training data and produces an inferred function, which can be used for predicting new examples (i.e., generalizing). One way to use SL in our problem would be to try to learn the general and \textit{true} WLAN behavior, function $f(x) = y$, through an estimate $h_\theta(x) = \hat{y}$, where $h_\theta(x)$ is the learned function. Then, once the hypothesis $h_\theta(x)$ is learned -- i.e., the error is sufficiently low with respect to $f(x)$ -- one could try to infer the input (or configuration) $\hat{x}^*$ that maximizes the performance $\hat{y}^*$, hoping that $\hat{x}^*$ would also result in the actual $y^*$.

The main three drawbacks of SL for our problem are \textit{i}) designing the model to fit, which should consist of a vast number of attributes (e.g., nodes' locations, configuration parameters, performance metrics, etc.), \textit{ii}) it needs a lot of data to learn accurate functions in complex systems (e.g., multi-parameter non-linear models), so our agents would not have that amount of time to do so,\footnote{We state that generating a dataset rich enough to generalize is unfeasible since data samples should have large multi-dimensional attributes to be meaningful. So, for instance, simply by moving one STA one meter away, a new scenario (or data sample) would be generated.} and \textit{iii}) SL is thought to generalize to unknown scenarios, %but this is not the focus of our problem because we want the agent to adapt to potentially infinite different worlds from scratch 
rather than indicating the agent how to adapt to the current one in real-time.
%\bcom{I don't understand this last point}\sergio{the idea was to emphasize that we don't care at all about the nature or model behind the system, i.e., we don't want to generalize. We simply want to get going as soon as possible} \bcom{Ok. Maybe just saying, "... unknown scenarios, rather than tell the agent how to adapt to the current one in real-time. }.
The only way to overcome such a task with SL would be to measure the performance of numerous settings in a lot of scenarios (primarily offline), then try to infer some general behavior from the true and unknown function $y = f(x)$, where input $x$ is the representation of the action setting and the environment around the agent, and finally predicting the performance $\hat{y} = h_\theta(x')$ for unlabeled (unknown) input $x'$. The significant issues are that the input domain of $x$ is multi-dimensional (with even categorical dimensions) and tends to infinity. The function $f$ representing WLANs' \textit{behavior} is so complex that learning an accurate estimate $h_\theta$ for realistic deployments is unfeasible.
%\bcom{too dramatic again!} \sergio{ok... but it is, right?} \bcom{It is... but sounds a bit strange. Unfeasible? or 'is hardly feasible' (just in case in some cases, it could be feasible)}

% Estimate is not the same as maximize
%Moreover, there is another issue when trying to replicate Wi-Fi through (deep) supervised learning: the problem of estimating a function is different from the problem of maximizing an unknown function. That is, even though we could get a good estimator $h_\theta(x)$ of the \textit{true} function, the optimal of such estimated function may be completely different than the \textit{true} optimal of $f$. In other words, our oracle may work well for most of the inputs $x$ but fail for the input $x^*$ maximizing $f(x)$.





%\cite{herzen2015learning} 

% -- Unsupervised Learning
%\subsubsection{Unsupervised Learning}
% What is UL
In \textbf{unsupervised learning} (UL), there are only inputs $x$ and no corresponding output variables. That is, there is no $y$. UL's goal is to model the underlying structure or distribution in the observed data to learn more about it. It is called unsupervised because, unlike SL there are no correct answers since samples are unlabeled. Algorithms are left on their own to discover potentially meaningful structures in the data. Clustering is the typical example of UL tasks.
%
Similarly to SL, the underlying structure of the observed data in the problem at issue is so complex that any attempt to model it through UL will be most likely fruitless. Hence, we believe that following an RL black-box approach is preferable: try to adapt from scratch to whatever the system's observations are, no matter its intrinsic nature.
% \bcom{This sounds good} \sergio{Great}

% ******************
% ******************





==> sections/old_sections_14Dec2020/rl_models.tex <==
\section{Reinforcement learning models}
% OLD

% Works on spectrum management using ML
Different ML solutions for the spectrum management problem, especially in RL, have been proposed in recent years.
% Why SoA works not good ---> common assumptions
However, certain assumptions these papers have in common hinder their accurate evaluation. For instance, most papers consider synchronous time slots (e.g., \cite{chen2020research}), a strong assumption that does not hold at all in WLANs. Also, some papers define a binary reward, where actions are simply good or bad (e.g., \cite{zhong2018actor}). This, while easing the RL framework, is not convenient for rewards taking into account continuous-valued performance metrics like throughput. Further, most of the papers consider fully backlogged regimes (e.g., \cite{nakashima2020deep}), thus overlooking the effects of factual traffic loads. To ease their analysis, some papers even consider conflict graphs rather than actual carrier sense areas (e.g., \cite{qi2020demand}), thus disregarding spatial distribution effects. Last but not least, a majority of the papers provide custom RL solutions that the reader may find complex to follow. Indeed, in most of cases, the design of states, actions, and rewards is not justified but simply formulated. This leaves short room to extrapolate such solutions to slightly different problems, making it also hard to reproduce the results.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.36\textwidth]{img/rl_diagram.pdf}
    \caption{RL diagram}
    \label{fig:rl_diagram}
\end{figure}

\subsection{RL approaches}
From the set of model-free RL approaches, we highlight MABs, Temporal Difference (TD) methods like Q-learning, and deep reinforcement learning (DRL).\footnote{We discard Monte Carlo methods since they require episodes to eventually terminate in order to work, which contrasts our vision of WLANs in continuous on-line adaptation in a so-called infinite episode.} Figure~\ref{fig:rl_types} depicts an schematized version of each of them in order of increasing complexity.

\begin{figure*}
    \centering
    \includegraphics[width=0.85\textwidth]{img/rl_types.pdf}
    \caption{Learning storage in MABs, Q-learning, and Deep Q-learning.}
    \label{fig:rl_types}
\end{figure*}

% - MABs
\subsubsection{Stateless RL variations}

The most common formulations of RL rely on states, which are mapped through a policy $\pi$ to an action $a$, i.e., $\pi(s) = a$. However, stateless approaches do also exist.
% Stateless
A key benefit of the stateless RL is precisely the absence of states, which eases its design by relying only on action-reward pairs. In this regard, the most representative stateless RL model for non-episodic problems is the MAB formulation.
% MAB
The MAB is a problem in which a fixed limited set of actions must be selected between competing choices to maximize expected gain. Each choice's properties are only partially known at the time of selection and may become better understood as time passes or by allocating resources to the choice \cite{sutton2018reinforcement}. MABs are a classic RL problem that exemplifies the exploration-exploitation trade-off dilemma.
% Stateless Q-learning
Apart from MABs, other works on wireless communications rely on a stateless Q-learning variation. %\bcom{A part del que va fer en Francesc?} \sergio{Yes, apart from Francesc's work.}

% - TD
\subsubsection{Temporal Difference}

% What is TD
TD learning is a combination of Monte Carlo and dynamic programming. Like Monte Carlo, TD can learn directly from raw experience without a model of the environment’s dynamics. Like dynamic programming, TD methods update estimates based on other learned estimates, without waiting for an outcome (i.e., they \textit{bootstrap}).
% SARSA And Q-learning
There are two main methods for TD: state–action–reward–state–action (SARSA) and Q-learning. SARSA and Q-learning work similarly, assigning values to state-action pairs in a tabular way. The key difference is that SARSA is on-policy, whereas Q-learning is off-policy. This means that SARSA learns action values relative to the behavior policy (or the policy it follows), while Q-learning does so by following a greedy policy. In other words, SARSA uses the value of the action following the same $\epsilon$-greedy policy all the time. In contrast, Q-learning uses the maximum value over all possible actions for the next iteration.

% - DRL
\subsubsection{Deep Reinforcement Learning}

% What is DRL
Deep learning (DL) is a branch of ML based on a set of algorithms that attempt to model high-level abstractions in data by using multiple processing layers, with complex structures or otherwise, composed of multiple non-linear transformations. They do so via deep neural networks (DNNs) consisting of multiple hidden layers. So, RL's combination with deep learning results in DRL, where the RL policy or algorithm uses a DNN rather than arrays or tables.
%
The most common form of DRL is a deep learning extension of Q-learning, called deep Q-network (DQN). So, as in Q-learning, the algorithms still work with state-action pairs, conversely to the MAB formulation. In plain, DQN is a much complex version of Q-learning. But why would one make the problem more complicated? It turns out that convergence in tabular Q-learning gets too slow when the number of states and actions increases. That is, it is so costly to keep gigantic tables that it is preferable to use DNNs to approximate such a table.

% --------------
% MABs
% ---------------
\subsection{Multi-Armed Bandits}   \label{sec:mabs}

% Why MABs
For most of the problems in uncoordinated wireless deployments like spectrum management, we propose having a MAB instance in each agent-empowered AP to adapt to the environment without states. The reason lies in the fact that meaningful states are intricate to define and its effectiveness heavily depends on the application and the type of scenario under consideration. In the end, a state is a piece of information that should help the agent by fitting it into its policy. If the state is meaningless, or worst, misleading, it is preferable not to rely on states and go for a stateless approach. In summary, when there is not plenty of time to train TD methods like Q-learning, it seems much better to go for a pragmatic approach: do gamble and find a satisfactory configuration as soon as possible, even though you will be most likely renouncing to an optimal solution.

% -----------------
% The MAB problem
% -----------------
\subsubsection{The MAB problem}

% Survey on MABs: https://arxiv.org/pdf/1904.07272.pdf

% What is a MAB
% From https://lilianweng.github.io/lil-log/2018/01/23/the-multi-armed-bandit-problem-and-its-solutions.html

% What is MAB
The multi-armed bandit problem is a classic RL problem that exemplifies the exploration vs. exploitation dilemma, where no knowledge on the reward probability distribution of each action is assumed.
% Example of MABs
The typical example to introduce the MAB problem is the gambler who faces multiple slot machines, each with different probability distributions over the money he/she can get after pulling the slots. Naturally, the gambler wants to get as much money as possible, thus achieving the highest reward in the mid/long-term. So, what strategy should he/she follow? That is where the MAB problem arises with its different variations. For instance, a naive approach would be to pull each machine slot a lot of times, so the gambler could guess the \textit{true} reward probability of each slot, and then select always the best slot machine. However, such an approach has obvious pitfalls like determining how many times are enough to discover the such a \textit{true} distribution or wasting too many trials (or iterations) in a priori lousy machines. Further, in environments where the distribution of such rewards may change due to external actors (as it is the case in WLANs), it would not be viable to get accurate estimates of the reward probability distributions. Simply because from one iteration to the other, the underlying reward distribution may be completely changed.

\subsubsection{Time horizon}
The duration imposed by the programmer to converge to a good solution determines the \textit{horizon}, which can be finite or infinite. Finite-horizon refers to when there is a need to perform (explore and exploit) during a given time window (e.g., 10 minutes). So, the number of iterations $T$ the agent counts with is finite. Thus, the RL algorithm must try to get the most accumulated reward with that ending in mind. Infinite-horizon, in contrast, poses no time limit to the agent to converge. For the spectrum management problem of this paper, we rely on finite horizons to assess the \textit{myopic} nature of the MABs. We call it myopic in the sense that they try to optimize rewards now without any explicit use of forecast information or any direct representation of decisions in the future. Meaning we want BSS's to improve its performance as soon as possible.

% -----------------
% Context taxonomy
% -----------------
\subsubsection{Contextual MABs}
%
While the general MAB formulation does not consider states, \textit{contexts} may be used to fine-grain the arm selection based not only on the gathered rewards, but also on further observations about the \textit{world}. In contextual bandits, reward distributions depend on a context, which is fit to the RL algorithm before making a decision. For instance, assume that an AP observes that a given basic channel, say basic channel 2, is busy most of the time. The derived context would then represent that channel 2 is active. Thus, it is not the same to apply the action corresponding to pick primary $p=2$ when the context indicates channel 2 is busy rather than applying the same action when such channel is idle. Henceforth, it seems that contexts may aid to the spectrum management problem, especially if we leverage knowledge from previous contexts (e.g., similar contexts stochastically repeated every day). However, contextual MABs also pose the challenge of appropriately defining contexts, meaning that a good representation of the environment should be captured in each context.

%\textit{Research choice}: So, should we go for a contextual bandit approach to tackle the joint spectrum management problem? We believe that it is better not to. Essentially, defining contexts may be as complex as defining states. And what would be an appropriate context definition? the current action? The current reward? A mix of the action selected and the reward? A mix including also historical information? Unfortunately, we do not identify any definition that suits our multi-agent and non-stationary reward problem. The reason lies in the fact that we want to boost the learning speed to raise the user experience in the short/mid-term. Then, relying on a different MAB per action in a contextual fashion would entail large and potentially unfruitful learning periods.

% -----------------
% Exploration algorithms
% -----------------
\subsubsection{The epsilon-greedy algorithm as a MAB} \label{sec:mab_exploration_algorithms}

The $\epsilon$-greedy or (e-greedy) algorithm, one of the simplest MAB formulations, takes the best recognized action with probability $1-\epsilon$, and explores a random action (previously explored or not) with probability $\epsilon$. The action value is estimated according to the past experience by averaging the rewards associated with the target action observed so far. In an exploring iteration, any action is picked with same probability, whereas in an exploitation iteration, the best known action is picked in a greedy way. We select $\epsilon$-greedy since it is one of the most well-known and simplest exploration algorithms for MABs. In particular, we set the initial exploration rate value to $\epsilon_0$=1, and decrease it after each iteration $t$ through the updating function $\epsilon=\epsilon_0/\sqrt{t}$, as suggested in~\cite{auer2002finite}.%\bcom{While in the other sections we justify why we focus on the contents, here not: we don't say why we talk now of the e-greedy.} \sergio{Ok, what about saying we select it as it is one of the simplest and best-known ones, so we use it as a MAB representative, the same way we use Q-learning as a TD representative?} \sergio{\textbf{Proposal made right before}} \bcom{ok}


==> sections/old_sections_14Dec2020/use_case.tex <==
\section{A use case on spectrum management}

% OLD

% -----------
% System model
% -----------
\subsection{System model and deployment}

% Explain deployment toy scenario
We study the deployment illustrated in Figure~\ref{fig:main_deployment}, consisting of $W =4$ potentially overlapping agent-empowered BSS's (with one AP and one STA each) in a system of 4 basic channels. The TMB path-loss model is assumed~\cite{adame2019tmb} and spatially distributed scenarios are captured. Namely, we cover scenarios where the BSS's may not all be inside the carrier sense range of each other. Therefore, the typical phenomena of home Wi-Fi networks like flow in the middle and hidden/exposed nodes are captured as in~\cite{barrachina2019dynamic}.
%
As for the action attributes, the primary channel can take any of the 4 channels in the system, $p\in \{1,2,3,4\}$, and the maximum bandwidth is allowed to be set to $b\in\{1,2,4\}$ fulfilling the 802.11ac/ax channelization restrictions for 20, 40, and 80 MHz bandwidths. So,  the total number of statuses when considering all BSS's to have constant traffic load raises to \mbox{$O(\mathcal{H}) = (4 \times 3)^4 = 20,736$}. Notice that even a petite deployment like this one leads to a vast number of possible statuses.\footnote{The 4-BSS's self-contained dataset for spectrum management in WLANs can be found at \url{https://www.upf.edu/web/wnrg/wn-datasets}.}

% Figure deployment toy scenario
\begin{figure}[h]
	%
	\centering
	\begin{subfigure}{0.255\textwidth}
		\includegraphics[width=\textwidth]{img/main_deployment.eps}
		\caption{Location of nodes.}
		\label{fig:main_deployment}
	\end{subfigure}
	~
	\begin{subfigure}{0.19\textwidth}
		\includegraphics[width=\textwidth]{img/interference_matrix.pdf}
		\caption{Interference matrix.}
		\label{fig:interference_matrix}
	\end{subfigure}
	
	\caption{Toy deployment of the self-contained dataset.}
	\label{fig:main_deployment_complete}
\end{figure}

% Justify complexity
The interference matrix elements in Figure~\ref{fig:interference_matrix} indicate the maximum %\bcom{or maximum? Maybe it's worth to say that for lower bandwidth values, they will still overlap}
bandwidth in MHz that causes two APs to overlap. So, we note that this deployment is complex in the sense that multiple different one-to-one overlaps appear depending on the distance and the transmission bandwidth in use, leading to exposed and hidden node situations hard to prevent beforehand. For instance, $\text{AP}_{\text{A}}$ and $\text{AP}_{\text{C}}$ can only overlap when using 20 MHz, whereas $\text{AP}_{\text{A}}$ and $\text{AP}_{\text{D}}$ do always overlap regardless of the bandwidth because their proximity. Instead, $\text{AP}_{\text{A}}$ and $\text{AP}_{\text{B}}$ overlap whenever 40 MHz (or 20 MHz) bandwidth is used.

% Dynamic channel bonding
We assume all the BSSs' have dynamic channel bonding capabilities to bond up to 4 basic channels. Nevertheless, the maximum number of channels to be aggregated is limited by the maximum bandwidth attribute $b$. For instance, we can easily restrict a BSS to single-channel transmissions by appropriately setting such attribute to $b=1$. Simulations are done through the Komondor wireless networks simulator~\cite{barrachina2019komondor}. The adaptive RTS/CTS mechanism introduced in the IEEE 802.11ac standard for dynamic bandwidth is considered and data packets generated by the BSS's follow a Poisson process with a mean duration between packets given by $1/\ell$, where $\ell$ is the mean load in packets per second. %\bcom{I think we can already introduce the load value}. 
In particular, we consider data packets of 12000 bits and all BSS's having a high traffic load $\ell = 50$ Mbps (or 4167 packets per second).
% Long-term traffic variations
%Unlike much of the works in the literature, we consider that the mean traffic load of every BSS may vary over time, thus introducing mid/long-term dynamism to the problem.

% Simulations
%To generate the self-contained dataset, we simulated all the possible statuses $\mathcal{H}$ of the deployment in Komondor~\cite{barrachina2019komondor}. So, we first create the deployment, meaning that we deploy the APs and STAs in fixed positions in the map (as in Figure~\ref{fig:main_deployment}). Then, we define the values of the modifiable attributes and the mean traffic load that each BSS experiences. Likewise, we set the configuration capabilities of each BSS, so we empower each agent with the action space $\mathcal{A}_w = \{\{p_w\},\{b_w\}\}$. For simplicity, we consider all the BSS's to have the same action space. Finally, for every WLAN's global configuration, we must generate all the input files corresponding to each possible status $\mathcal{H}$ to be later simulated with Komondor. Notice that the input $x = \mathcal{H}$ is mapped to the output $y$, where $y$ is an array containing multiple performance metrics of each BSS, including throughput and delay. Every status $\mathcal{H}$ is evaluated during $T_{\mathcal{H}} = 5$ seconds. Given that the WLAN remains steady during any status, we empirically found that 5 seconds is enough to accurately estimate the long-term mean performance. We use Wi-Fi parameters according to 802.11ax \cite{barrachina2019online}.

% Traffic patter and ML
%Once we gather the whole dataset of the deployment through Komondor, we use it to benchmark the performance of the MAB algorithms depicted in \S\ref{sec:mab_exploration_algorithms} under different traffic patterns. For the sake of explanation, assume that the WLAN starts at $t_0 = 0$ with status $\mathcal{H}_0$. At $t_1$, one agent-empowered BSS picks an action $a_1$ (e.g., switches the primary channel), leading to status $\mathcal{H}_1$. Notice that, since we already have the dataset generated, it is straightforward (and fast) to check the performance $y$ of all the BSS's in the WLAN at such given status. We essentially use the dataset as a lookup table $x= \mathcal{H} \rightarrow y$, so the computation speed rises.

% - Benchmarking RL algorithms
\subsection{Benchmarking RL approaches}

% Research question
Part of the reasoning we conducted on why MABs seemed the most suitable approach was related to the fact of avoiding states. This way, there is no need to seek meaningful state definitions, and the learning can be executed more quickly since only actions and rewards are used to execute the policy. Nonetheless, in this experiment, we go beyond such qualitative reasoning and provide a quantitative measure on Q-learning performance (relying on states), and contextual MABs (relying on contexts).

\subsubsection{State and context spaces}

\begin{figure}[h]
    \centering
    \includegraphics[width=0.4\textwidth]{img/state_spaces.pdf}
    \caption{Binary and combined state spaces.}
    \label{fig:state_spaces}
\end{figure}

We propose two state and context space definitions as shown in Figure~\ref{fig:state_spaces}. The smaller state space is 1-dimensional and relates exclusively to the throughput satisfaction and is binary, i.e., it is composed of the satisfied and unsatisfied states. That is, if all the packets are successfully transmitted, the BSS is satisfied ($s=1$), and unsatisfied otherwise ($s<1$).
% Second state space
The larger state space is 3-dimensional, and results for the combination of the binary throughput satisfaction and the action attributes (primary $p$ and max bandwidth $b$). So, the state space raises from 2 to 24 states, corresponding to the combination of 2 binary throughput satisfactions, 4 primary channels, and 3 maximum bandwidths.

These state definitions contain key parameters as for the Wi-Fi domain knowledge: \textit{i}) being satisfied or not is critical to user experience, and \textit{ii}) the spectrum configuration (or action) is most likely affecting the BSS performance. %\bcom{Do they provide information of the environment? They only provide information about the BSS...} 
%\bcom{Can we find any motivation in defining these states? I'm sure reviewers will ask for that justification.} \sergio{\textbf{Proposal made right before}} \bcom{I would not give readers the opportunity to think if the states provide not much info (if they don't do by themselves), i.e., removing that sentence where we say that. I would just be positive when introducing the states. Note that the considered states take into account critical aspects that impact the decisions that the agent may take.} 
As for the former, being satisfied is actually the goal of the RL problem, so it will highly condition the action selection. Similarly, the current action seems a good indicator for suggesting which the next one should be.
% Problem with larger states
Notice that higher multi-dimensional state definitions considering parameters like spectrum occupancy statistics would exponentially increase the state space, thus being cumbersome to explore and consequently reducing the learning speed dramatically.\footnote{From this brief discussion on the size of the state-action space we can conclude that more complex approaches like DRL do not suit the problem of this paper since DRL relies on huge state-action spaces and normally takes long periods to start learning.}

% Q-learning and contextual
To assess the convenience of states or context we use Q-learning and a contextual formulation of $\epsilon$-greedy. Q-learning is a temporal difference algorithm seeking the best action to take given the current state. It is considered off-policy because the Q-learning function learns from actions outside the current policy, like taking random actions. The learning rate $\alpha$ or step size determines to what extent newly acquired information overrides old information. A factor $\alpha = 0$ makes the agent learn nothing (exclusively exploiting prior knowledge). In contrast, a factor $\alpha = 1$ makes the agent consider only the most recent information (ignoring prior knowledge to explore possibilities). We use a high value of $\alpha = 0.8$ because the non-stationary of the multi-agent setting. The discount factor $\gamma$ determines the importance of future rewards. A factor $\gamma=0$ will make the agent myopic (or short-sighted) by only considering current rewards, while a factor approaching $\gamma \rightarrow 1$ will make it strive for a long-term high reward. We use a relatively small $\gamma = 0.2$ to foster exploitation (for rapid convergence) in front of exploration.

% Contextual MAB
Another way in which agents use partial information gathered from the environment is in the form of contexts. In plain, contexts can be formulated as \textit{states for stateless approaches}. That is, a contextual MAB can be instantiated like a particular MAB running separately per context. The learning is separated from one context to the other so that no information is shared between contexts like it is the case for Q-learning and other state-full approaches. In this case, we define the contexts as the states and propose having a separate MAB instance for each of the contexts.


\subsubsection{Evaluation}

% Simulations
% Methodology
We assume each BSS having a the same traffic load, $\ell = 50$ Mbps. So, this experiment's long-term dynamism is due exclusively to the multi-agent setting. %\bcom{Is because the load is constant, not because is high, as it could be understood here} 
That is, the inner traffic load conditions do not vary, but the spectrum management configurations (or actions) do. For the sake of assessing the learning speed, we consider a relatively short time-horizon of 200 iterations, each of 5 seconds. We run 100 simulations for each RL algorithm.

\begin{figure}[h]
    \centering
    \includegraphics{img/evaluation.eps}
    \caption{Run chart of the normalized cumulative gain for the worst BSS and WLAN's mean, averaged over 100 simulations. The number within the brackets in the contextual and q-learning terms refers to the context/state space size.}
    \label{fig:evaluation}
\end{figure}

% Results
% Thrsat performance
Figure~\ref{fig:evaluation} shows the normalized cumulative reward $G_{w,t}/t$ averaged trough the 100 simulations for the worst-performing BSS and the WLAN's mean. We also show the optimal value, which turns out to be 1 for the worst and mean value since there exist few global configurations where all the BSS's are satisfied. %\bcom{Not sure to understand what do you mean with this sentence... is 1 because all WLANs are fully satisfied with the optimal configuration all the time?} \sergio{\textbf{Proposal made}}
We plot 5 curves in each subplot corresponding to the different RL approaches: raw $\epsilon$-greedy, contextual $\epsilon$-greedy for the binary and combined contextual spaces, and Q-learning also for the binary and combined state spaces.
% We observe
We observe that while $\epsilon$-greedy converges (learns) to higher reward values close to the optimal, the rest context/state-aided algorithms learn much slowly, way below $\epsilon$-greedy's performance. In particular, the MAB is able to get a near-optimal mean performance (just 7\% away for complete satisfaction). This relates to the fact that learning based on states/contexts is fruitless in dynamic and chaotic multi-agent deployments like this. So, it seems preferable to act quickly with a lower level of world awareness.
% Fairness
Besides, we note that the MAB is able to establish win-win relations between the BSS's, as shown by the worst performing BSS subplot. That is, on average, BSS's tend to benefit from others' benefits, resulting in fairer configuration. In particular, outperforms the worst-case performance more than 30\% with respect to the rest algorithms.

% Comparison within states
In fact, we observe that both Q-learning and the contextual MAB formulation perform better when relying on the binary state/context space definition. That is, by shrinking the state space from 24 to 2 the learning speed raises up. So, rather than aiding the learning, extensive state space slow down the learning, taking much more time to be explored. Further, by eliminating the states and relying on the MAB, the performance is significantly improved. This use-case showcases the MAB's ability to learn in multi-agent Wi-Fi deployments by establishing win-win relationships between BSS's.
%\bcom{Even if it is not for the paper, but I would like to understand what kind of world awareness offer the states in this case}. \bcom{I like this win-win relation concept}. \sergio{Ok, we can think about it}


